WearableMil: An End-to-End Framework for Military Activity Recognition and Performance Monitoring

Musculoskeletal injuries during military training significantly impact readiness, making prevention through activity monitoring crucial. While Human Activity Recognition (HAR) using wearable devices offers promising solutions, it faces challenges in processing continuous data streams and recognizing diverse activities without predefined sessions. This paper introduces an end-to-end framework for preprocessing, analyzing, and recognizing activities from wearable data in military training contexts. Using data from 135 soldiers wearing \textit{Garmin--55} smartwatches over six months with over 15 million minutes. We develop a hierarchical deep learning approach that achieves 93.8% accuracy in temporal splits and 83.8% in cross-user evaluation. Our framework addresses missing data through physiologically-informed methods, reducing unknown sleep states from 40.38% to 3.66%. We demonstrate that while longer time windows (45-60 minutes) improve basic state classification, they present trade-offs in detecting fine-grained activities. Additionally, we introduce an intuitive visualization system that enables real-time comparison of individual performance against group metrics across multiple physiological indicators. This approach to activity recognition and performance monitoring provides military trainers with actionable insights for optimizing training programs and preventing injuries.

==> files/7-Discussion.tex <==
Our framework reveals key trade-offs in wearable-based military activity recognition: longer windows provide richer context but may miss brief critical events like ``Wake Up'' (20 min) or short ``Running Exercise'' sessions essential for assessing training intensity and recovery. The framework enhances military training monitoring by: (1) supporting individualized training through real-time visualization of individual versus group performance for training optimization and injury prevention, and (2) reducing unknown states from 40.38\% to 3.66\% via physiologically-informed sleep imputation, enabling comprehensive recovery analysis crucial for soldier readiness. Limitations include: reliance on statistical HR calculations rather than ML methods, potentially limiting generalizability without extensive historical data; fixed windows (45-60 min) potentially missing short-duration activities; and technical challenges from sensor inaccuracies and device removal during specific activities (e.g., ``Contact-Combat,'' 48.5\% accuracy), highlighting needs for improved data collection strategies.

==> files/OLD-2-relatedwork.tex <==
HAR in group training settings utilizes advanced methods to identify activities conducted by groups rather than individuals, posing distinct difficulties in understanding collective actions. The utilization of hybrid techniques, such as the multilayer perceptron neural network in conjunction with IMU sensors, has exhibited remarkable precision in discerning specific activities by enhancing sensor data and employing Fast Fourier transform for feature extraction \cite{mao2023hybrid}. DL frameworks, specifically those that use graphical models, have been used in group settings to analyze the interactions between group members. These frameworks aim to capture both the actions of individuals and the overall behavior of the group \cite{salian2023group}. The active factor graph network model expands upon conventional second-order interactions to incorporate third-order interactions, thereby offering a more nuanced comprehension of group dynamics by taking into account the impact of pivotal individuals within the group \cite{xie2024active}. In addition, transfer learning models that utilize CNN architectures such as ResNet and MobileNet have achieved success in accurately identifying various activities by employing efficient feature extraction and majority voting fusion techniques \cite{jannat2023human}. Furthermore, the integration of multiple modes of wearable data provides an additional aspect to HAR. 

Injury prediction using HR, steps, and sleep data entails combining biometric and activity metrics to predict potential injury risks. Predictive modeling is crucial in diverse fields such as sports and healthcare, as it enables timely intervention to avert serious consequences. A recent study employed ML methods to analyze heart rate variability (HRV) and found that spectral analysis of HRV can accurately forecast trauma outcomes. This indicates that these physiological measurements play a crucial role in evaluating the severity of injuries and predicting the course of recovery \cite{luo2021spectral}. In \cite{kleinsasser2022detecting} a study was conducted to examine the use of wearable devices such as Fitbits to predict sleep patterns. The study achieved a high level of accuracy in predicting sleep patterns and also demonstrated the potential for predicting other health-related events, such as injuries. In addition, ML models utilized on runners' training logs, which include measurements such as steps taken and subjective effort, demonstrated a good ability to accurately predict injuries. This was especially evident when analyzing the training intensity leading up to the occurrence of injuries \cite{lovdal2021injury}. Those findings of these studies suggest that the integration of HR, steps, and sleep data with advanced enough ML algorithms can establish reliable frameworks for predicting injuries.

Our work integrates wearable sensor data with ML to identify and analyze group training activities. We extend previous research by focusing on collective dynamics in military training, addressing missing data primary of sleep data, while utilizing multiple data streams. 




%% \begin{table}[t]
% \centering
% \caption{Performance Comparison: Temporal vs. User Splits}
% \label{tab:split_comparison}
% \begin{tabularx}{\columnwidth}{lXXXXX}
% \toprule
% \textbf{Split Type} & \textbf{Accuracy  (L1)} & \textbf{F1 (L1)} & \textbf{AUC (L1)} & \textbf{F1 (L2)} & \textbf{AUC (L2)} \\ \midrule
% Temporal           & 93.8\%               & 93.8\%          & 95.3\%               & 74.0\%          & 84.1\%               \\
% User               & 83.8\%               & 83.8\%          & 87.6\%               & 66.5\%          & 79.0\%               \\ \bottomrule
% \end{tabularx}
% \end{table}


==> files/OLD-3-evaluating-ML-models.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{files/figs/HARpipeline.pdf}
    \caption{Overview of the Data Processing and Prediction Pipeline. The pipeline integrates multi-source wearable data, including heart rate, physical activity, and sleep data, into a unified grid using both a linear truncated model (LTM) and epoch-based aggregation. Missing sleep data is imputed leveraging physiological insights and physical activity thresholds. Windows of varying sizes are labeled and inputted into an LSTM network, which captures sequential dependencies to predict activities over predefined time intervals. }
    \label{fig:pipeline}
\end{figure}
Figure~\ref{fig:pipeline} shows the main stages of the proposed framework. In the first stage, HR data is used to compute personalized metrics that assist in managing the various sampling frequencies of the data. In Stage 2, these metrics are applied to project the different data modalities onto a common time grid. Stage 3 involves segmenting the features into windows suitable for input into the LSTM model, which is trained to predict outcomes. Each stage is described in detail below.

\textbf{Data Collection and preprocessing} Between September 4, 2022, and March 1, 2023, 135 soldiers wore the same smartwatch, Garmin 55, while living together and following a consistent daily schedule. \footnote{Each participant signed an inform consent after an explanation about the study and volunteered to the study. The study was approved by Helsinki committee of the IDF’s Medical Corps ethical board (1998-2019) and by the Human Use Committee of Sheba Medical Center (6333-19-SMC)}. The collected dataset comprises all the raw data provided by Garmin, as specified in the Health REST API Specification \cite{garmin_health_api}. The primary data points we consider include heart rate (HR), epoch data (containing steps and distance covered), and sleep-related data. In the following section, we describe in detail the preprocessing steps applied to each of these subdomains, in order to combine them together using the same time grid. 

\textbf{Preprocessing heart rate measurements}
Garmin watches utilize photoplethysmography (PPG) sensors to monitor HR. These sensors operate by emitting light into the skin and detecting the amount of light absorbed or reflected back by the blood vessels. Variations in blood volume, caused by the heart's pumping action, lead to fluctuations in light absorption, which the sensors capture to determine HR. This is a non-invasive technique. For HR data collection, Garmin wearables record measurements at intervals of every 15 seconds. We downsampled these measurements to a one-minute interval by averaging the pulse across every four samples.

Prior to downsampling, we calculated the minimum and maximum HR values for each day by identifying the 5th and 99.98th percentiles for each soldier. We then aggregated these daily values across the entire dataset to determine the median minimum and maximum HR for each individual referred to as \textit{minHR} and \textit{maxHR}. These metrics were then used to fill in gaps in the sleep data and accurately compute distances and steps taken during specific time intervals, as outlined below and shown in figure \ref{fig:pipeline}. This approach enables us to assess the relative effort exerted by each soldier based on their personalized HR metrics.

\textbf{Preprocessing epoch measurements}
Garmin watches record distance covered and steps taken using a combination of accelerometer data and GPS tracking. The accelerometer estimates steps by measuring wrist movements and detecting changes in acceleration along different axes. However, when the arm is motionless or performing tasks that do not produce distinct movements, such as pushing a cart, this method may occasionally miss steps. GPS tracking is not utilized unless a specific activity is activated. Consequently, the watch relies solely on integrated sensors, such as the accelerometer, to estimate metrics like steps and distance, using either a standard or user-defined step length instead of actual GPS data.

The wearables collect measurements every 15 minutes for epoch data collection. To understand a person's behavior on a per-minute basis in terms of steps and distance covered, we introduce two strategies: the Linear Truncated Model (LTM) and the Exponential Model (EM). These models ensure that HR, steps, and distance covered are all aligned on the same grid.

\textit{Linear Truncated Model}: The LTM provides a straightforward approach that linearly correlates HR with physical activity metrics such as distance and steps. In this model, we use the \textit{minHR} parameter calculated for each individual, considering only data points where the pulse rate exceeds this threshold, multiplied by a factor of $1.1$. Each minute's contribution within a 15-minute interval is directly proportional to the pulse rate, with higher pulse rates resulting in proportionally greater contributions.

\textit{Exponential Model}: The EM, on the other hand, employs a non-linear approach by exponentially weighting each minute's contributions based on the pulse rate. Like the LTM, the \textit{minHR} threshold is used to filter out low-activity periods. However, above this threshold, the model disproportionately emphasizes higher pulse rates using an exponential function. This method is particularly beneficial for highlighting high-intensity activities, as it reflects the increased effort associated with higher pulse rates. The exponential weighting can more accurately capture the rapid escalation in physical output as intensity increases, which may not be as apparent in a linear model.
\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{files/figs/LTM_1.pdf}
        \caption*{(a) Linear Truncated Model }
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{files/figs/EXP_1.pdf}
        \caption*{(b) Exponential Model}
    \end{minipage}
    \caption{Time-series modeling comparing two different models during a fitness test. Figure (a) presents the output from the LTM, while Figure (b) shows the results from the EM. Both graphs depict the distance covered in meters, steps, and the pulse ratio relative to the minimum HR throughout the fitness test, which originally was in 15-minute interval. The left y-axes represent the distance (meters) and steps, while the right y-axis indicates the pulse ratio to minimum HR, which serves as a measure of cardiovascular effort relative to the individual's baseline.}
    \label{fig:comparisonEMvsLTM}
\end{figure}

Figure~\ref{fig:comparisonEMvsLTM} compares the same soldier's fitness test data processed by the LTM and the EM. The figure shows (a) the LTM versus (b) the EM. In each plot, the left axis represents distance and steps, while the right axis corresponds to the pulse ratio relative to the \textit{minHR}. The LTM provides a steady view of overall activity, aligning with the left axis, while the EM highlights intensity spikes, particularly on the right axis, where the exponential weighting emphasizes bursts of exertion. This contrast shows how the EM brings out high-intensity activities, whereas the LTM offers a more balanced depiction of sustained physical activity. Therefore, for evaluating, we use only the LTM model and do not use EM.

\textbf{Preprocessing sleep measurements} Garmin watches utilize built-in sensors to monitor various aspects of sleep, offering a comprehensive overview of a user's sleep quality and patterns. The data collected encompasses the duration and different stages of sleep, including light, deep, and REM sleep, as well as periods of wakefulness. These insights are derived from continuous tracking of movement and HR variability, allowing the device to accurately detect transitions between various sleep stages.

The collected data includes the duration and stages of sleep, such as light, deep, and REM sleep, as well as periods of wakefulness. These findings are derived from continuous monitoring of movement and HR variability, enabling the device to detect transitions between different sleep stages. 

To prepare the data for analysis, we first transformed the sleep stages, which are typically recorded within specific hour ranges, into one-minute intervals for each individual, assigning an associated category to each interval. For minutes without recorded data, we initially assigned a ``?'' to indicate missing data. Since Garmin watches do not track sleep during the day, we developed a method to intelligently impute missing data points both at night and during the day, allowing us to account for daytime sleep periods.

To impute missing data during the night, we utilized \textit{minHR}. If a soldier's pulse rate was below \textit{minHR} and they had recorded zero steps during a given minute,that minute was labeled as sleep. For daytime hours, we adjusted the threshold, using a condition of pulse$\leq$$\textit{minHR}\cdot 1.10$ to determine sleep. This allows us to impute missing data points, which we then verified against the planned schedule.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{files/figs/sleep_impute6.pdf}
    \caption{Visualization of sleep states and HR data before and after processing of a week time of a single soldier. The top part of the figure shows sleep states categorized as ``Awake'' ``Sleeping'' and ``Unknown'' before processing, and as ``Awake'' ``Sleeping'' and ``Not Enough Info'' after processing. The bottom part depicts HR data over the same time period, displaying fluctuations in heart rate across multiple days. The imputation process is reflected in the adjusted sleep states, providing a clearer distinction between sleep phases and periods of insufficient data.}
    \label{fig:sleep}
\end{figure}

Additionally, we applied a second imputation technique using extrapolation. This involved identifying instances where five consecutive minutes had the same recorded value followed by a ``?'' and filling in the missing data with the value from the previous measurements. Finally, we categorized the data into three categories: ``0'' for awake, ``1'' for sleep, and ``2'' for unknown data points. 

Figure~\ref{fig:sleep} presents a side-by-side comparison of sleep state classification and HR data before and after imputation for the week starting on December 11, 2022. The visualization is divided into two sections. On the left, sleep states before processing display the original classification of sleep states, categorized as Awake (red), Sleeping, which includes light sleep, deep sleep, and REM, as recorded on the watch (green), and Unknown (grey), representing periods where the sleep state was not determined by the watch. On the right, sleep states after processing show the results after imputation, where unknown states have been reclassified as either Awake (red), Sleeping (green), or marked as Not Enough Info (grey), indicating periods where data is still insufficient even after processing. The x-axis represents time, spanning from December 5, 2022, to December 12, 2022, while the y-axis in lower plots represents HR. The HR data (red line) provides context on the individual's physiological state during this period, while the horizontal dashed line is this specific soldier's calculated \textit{minHR} value. Notably, after imputation, gaps in sleep state classification are significantly reduced, with fewer unknown periods. This illustrates how the imputation process refines the data, filling in missing or uncertain sleep states, resulting in a more continuous and accurate representation of the individual's sleep patterns.

\begin{table}[h!]
\centering
\begin{tabular}{lccc}
\hline
\textbf{Metric} & \textbf{Pre-processing Averages} & \textbf{Post-processing Averages} & \textbf{Difference (Post - Pre)} \\ \hline
Amount of data in minutes       & 78598.03  & 78598.03  & 0.00   \\ 
Amount of filled sleep data      & 15034.03  & 41789.06  & 26755.03  \\ 
Amount of filled awake data      & 610.66    & 35771.93  & 35161.27  \\ 
Amount of missing data           & 62953.34  & 1037.05   & -61916.29 \\ 
Percent of data filled           & 18.44     & 95.11     & 76.67\%    \\ 
Percent of data missing          & 81.56     & 4.89      & -   \\ \hline
\end{tabular}
\caption{Comparison of pre- and post-processing averages, including the difference between post- and pre-processing values.}
\label{table:sleeping}
\end{table}

Table \ref{table:sleeping} highlights the differences between the pre-processing and post-processing averages for the key metrics related to the completeness and quality of the sleep data. Before processing, the data contained a significant amount of missing information, with an average of 81.56\% of the data being unfilled. We consider a data point as one minute. After applying our imputation techniques, the percentage of filled data increased dramatically from 18.44\% to 95.11\%, reflecting an improvement of 76.67\%. Similarly, the amount of filled sleep data increased by 26,755.03 minutes (\textbf{about 18 days}), while the amount of filled awake data saw an even larger increase of 35,161.27 minutes (\textbf{about 24 days}). Conversely, the amount of missing data decreased significantly by 61,916.29 minutes. These results demonstrate the effectiveness of the imputation process in enhancing data completeness, thereby reducing the impact of missing data and allowing for more reliable insights into sleep behaviors. The appendix provides the data for each individual. 

\textbf{Dataset creation} To apply supervised learning to time series data, it is essential to transform the data into input-output pairs. For this purpose, we employed the sliding window technique \cite{frank2001time}, which requires specifying two parameters: the sliding window length and the sliding step. In our case, we used sliding window lengths of 30 and 60 minutes, resulting in training samples with 30 and 60 rows of multiple features, respectively. During training, we applied a 90\% overlap between consecutive windows, corresponding to 27 and 54 minutes, to maximize the number of training samples. Since the data labels are derived from the soldiers' schedules, the labels differ in both length and timing. For a label to be assigned to a specific window, it must be continuous for at least the duration of the window (either 30 or 60 minutes). This ensures that each window in the dataset is accurately labeled according to the corresponding schedule.

\textbf{Evaluating the models} To illustrate the practical capabilities of our models, we first show an evaluation using an 80:20 train-test split, where 80\% of the data was utilized for training and the remaining 20\% was reserved for testing on out-of-sample data. This initial evaluation allowed us to assess the model's generalization capabilities. In the following section, we further extend the evaluation to include out-of-sample days, providing a more comprehensive analysis of the model's performance. The dataset used for these evaluations is based solely on heart-rate and epoch-related data to identify various activities. For sleep identification, we provide statistics on the successful imputation of sleep times, achieved without the use of machine learning techniques.

The input data was preprocessed as described earlier and further segmented into sequences of features using a sliding window approach. To mitigate class imbalance within the dataset, we applied the Synthetic Minority Over-sampling Technique (SMOTE) \cite{chawla2002smote}, a widely recognized method for generating synthetic instances of minority classes. By augmenting the dataset with these additional examples, SMOTE effectively balanced the training data, thereby improving the model's ability to accurately classify activities that were previously underrepresented.

The ML model's architecture is based on a Long Short-Term Memory (LSTM) network \cite{yu2019review}, which excels at processing sequential data. The input layer is designed to handle five key features: \textit{pulse, steps per minute, distance covered per minute, pulse min ratio, and pulse max ratio}. The pulse min and max ratios were computed during preprocessing by dividing the pulse for each minute by the respective \textit{minHR} or \textit{maxHR} values. In the windowed dataset, timestamps are intentionally excluded, as the windows represent relative time intervals of 30 or 60 minutes, ensuring the model focuses on activity recognition without being tied to specific times. After the input layer, which extracts relevant features while preserving the temporal sequence, LSTM layers are utilized to capture the inherent temporal dependencies in the data. The model concludes with a fully connected output layer that translates these learned temporal patterns into activity classifications. The architecture includes two LSTM layers, each containing 64 neurons.

The model was trained with a batch size of 32, using the Adam optimizer~\cite{kingma2014adam} and the ReduceLROnPlateau learning rate scheduler. This scheduler tracks the validation loss and reduces the learning rate by 50\% when a plateau is detected, allowing for finer adjustments during training. To prevent overfitting, early stopping was applied, with a patience of ten epochs, meaning training was stopped if the validation loss did not improve over ten consecutive epochs. After training, the model was evaluated on a test set, which constituted 20\% of the original dataset. The evaluation involved comparing the predicted labels with the true labels to assess model performance.

\begin{figure}[t]
    \centering
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{files/figs/OOS_30reg.pdf}
        \caption*{(a) 30-minute window length}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{files/figs/OOS_60regloaded.pdf}
        \caption*{(b) 60-minute window length}
    \end{minipage}
    \caption{Confusion matrices comparing the performance of activity recognition models using two different sliding window lengths.  (a) presents the results for the 30-minute window length, while (b) shows the results for the 60-minute window length. The matrices display the predicted activities on the x-axis and the true activities on the y-axis. The color shading reflects the proportion of correct and incorrect predictions, with darker shades representing higher values. The bar on the right shows the corresponding color scale for the prediction proportions.}
    \label{fig:confusionMat}
\end{figure}

Figure~\ref{fig:confusionMat} presents two confusion matrices for two different sliding window lengths of 30 minutes and 60 minutes, respectively, for the same set of activities. The matrices shows the models' performance in predicting each activity, highlighting how the choice of window length impacts classification accuracy. Each matrix is normalized to show the percentage of predictions. The color intensity within each matrix reflects the proportion of correctly and incorrectly classified instances, allowing for a direct comparison between the two window lengths in terms of model accuracy across the activities.

Figure~\ref{fig:confusionMat}(a) shows that the model trained with a 60-minute sliding window length generally exhibits higher accuracy across most activities compared to the model trained with a 30-minute window. For example, the accuracy for ``Everyday Activity'' with the 60-minute model is 82.28\%, significantly outperforming the 62.53\% accuracy achieved by the 30-minute model. This trend is consistent across activities such as ``Rifle Drill'' where the 60-minute model achieves an accuracy of 70.18\%, compared to 55.91\% for the 30-minute model. The rest of the activies bbetween the two window lengths are comparable. Lastly, the 60-minute model shows a marked improvement in reducing misclassification, as seen in the lower percentages of confusion between similar activities. These results indicate that while the 60-minute model is generally more accurate, the 30-minute model could still be preferable for specific, more detailed activity recognition tasks, that are generally known to be shorter. We can see that using a 30-minute window length, we have activities such as ``Obstacle Training'' that do not exist in the 60-minute window, since they do not take more then 60-minute, therefore those do not have a label when using a 60-minute sliding window.

==> files/check111.tex <==
\textbf{Clustering Quality and Validation.}
For DNA storage applications, clustering accuracy must satisfy stricter requirements than traditional classification metrics. Following~\cite{rashtchian2017clustering}, we define clustering accuracy in terms of the overlap between predicted clusters $\tilde{C}$ and ground truth clusters $C$. Formally, for an alphabet $\Sigma = \{A,C,G,T\}$ representing the four DNA nucleotides, and strings $x,y \in \Sigma^*$, the edit distance $d_E(x,y)$ equals the minimum number of insertions, deletions, or substitutions needed to transform $x$ to $y$. The distance between two nonempty sets $C_1, C_2 \subseteq \Sigma^*$ is defined as:
\[
d_E(C_1,C_2) = \min_{x \in C_1, y \in C_2} d_E(x,y)
\]

For a clustering $C$ of DNA sequences, the accuracy $\mathcal{A}_{\gamma}(C, \tilde{C})$ measures the quality of predicted clusters $\tilde{C}$ relative to ground truth $C$:
\[
\mathcal{A}_{\gamma}(C, \tilde{C}) = \max_{\pi} \frac{1}{|C|} \sum_{i=1}^{|C|} \mathbf{1}\{\tilde{C}_{\pi(i)} \subseteq C_i \text{ and } |\tilde{C}_{\pi(i)} \cap C_i| \geq \gamma|C_i|\},
\]
where $\gamma \in (\frac{1}{2},1]$ represents the required fraction of overlap and $\pi$ is an injective mapping $\pi: \{1,2,...,|C|\} \rightarrow \{1,2,...,\max(|C|,|\tilde{C}|)\}$. This formulation ensures that each predicted cluster contains a substantial portion of exactly one ground truth cluster while prohibiting false positives.

Our signal-model achieves robust performance across standard metrics, with Rand scores consistently exceeding 0.88 and reaching 0.971 and 0.978 for the \emph{Microsoft Experiment} and \emph{Deep DNA Test} datasets, respectively. To ensure cluster quality specifically for DNA storage applications, we implement two additional validation criteria derived from the theoretical accuracy definition:

\begin{enumerate}
   \item \textbf{Dominant Label Criterion:} For each cluster $\tilde{C}_i$ with dominant label $l_i$, we require:
   \[
   \frac{|l_i \in \tilde{C}_i|}{|N_i|} \geq \gamma, \quad \gamma = 0.6
   \]
   where $|l_i \in \tilde{C}_i|$ denotes the count of label $l_i$ in cluster $\tilde{C}_i$, and $|N_i|$ represents the total count of label $l_i$ in the dataset. This criterion ensures sufficient coverage of each ground truth cluster.

   \item \textbf{Minority Label Constraint:} For all labels $l_j \neq l_i$:
   \[
   \frac{|l_j \in \tilde{C}_i|}{|\tilde{C}_i|} \leq \beta, \quad \beta = 0.2
   \]
   This constraint enforces cluster purity by limiting contamination from other classes to a fraction $\beta$ of each cluster's size.
\end{enumerate}

These criteria align with the theoretical requirements for DNA storage retrieval, where each cluster must reliably represent a distinct stored information unit. The choice of $\gamma = 0.6$ ensures majority representation while accommodating noise inherent in DNA sequencing, while $\beta = 0.2$ provides a strict bound on cluster contamination. This formulation generalizes the standard classification error metrics while providing stronger guarantees needed for DNA storage applications.




% @article{rashtchian2017clustering,
  % title={Clustering billions of reads for DNA data storage},
  % author={Rashtchian, Cyrus and Makarychev, Konstantin and Racz, Miklos and Ang, Siena and Jevdjic, Djordje and Yekhanin, Sergey and Ceze, Luis and Strauss, Karin},
  % journal={Advances in Neural Information Processing Systems},
  % volume={30},
  % year={2017}
}
